Diffuse TeV Emission at the Galactic Centre

The High-Energy Stereoscopic System (HESS) has detected intense diffuse TeV emission correlated with the distribution of molecular gas along the galactic ridge at the centre of our Galaxy. Earlier HESS observations of this region had already revealed the presence of several point sources at these energies, one of them (HESS J1745-290) coincident with the supermassive black hole Sagittarius A*. It is still not entirely clear what the origin of the TeV emission is, nor even whether it is due to hadronic or leptonic interactions. It is reasonable to suppose, however, that at least for the diffuse emission, the tight correlation of the intensity distribution with the molecular gas indicates a pionic-decay process involving relativistic protons. In this paper, we explore the possible source(s) of energetic hadrons at the galactic centre, and their propagation through a turbulent medium. We conclude that though Sagittarius A* itself may be the source of cosmic rays producing the emission in HESS J1745-290, it cannot be responsible for the diffuse emission farther out. A distribution of point sources, such as pulsar wind nebulae dispersed along the galactic plane, similarly do not produce a TeV emission profile consistent with the HESS map. We conclude that only a relativistic proton distribution accelerated throughout the inter-cloud medium can account for the TeV emission profile measured with HESS.

==> readme <==
DiffuseTeV.tar.gz contains 16 figures in encapsulated postscript (eps) form
which combine to create 9 total figures in the paper ms.rev.tex

No special formatting needs to be done for the figures although I 
found that the command "latex ms.rev.tex" needed to be done twice; 
otherwise, references to figures (e.g. \ref{fig:coolingrates}) were 
not recognized.

